A mechanistic characterization of missingness at random

The missingness-at-random (MAR) assumption underlying many missing-data methods describes abstract statistical independences, whereas practitioners reason more naturally about the causal mechanisms that generate missingness. To bridge this gap, we provide a mechanistic characterization of MAR in terms of paths in a directed acyclic graph (DAG) modified to allow certain edges to cease to operate when an incomplete variable is missing, a property termed "context-specific causal irrelevance (CSCI)". Under a faithfulness condition, MAR holds if and only if the modified DAG contains no MAR-violating paths. Without CSCI, this condition reduces to a previously established d-separation condition, VMAR; thus, MAR without VMAR requires specific kinds of CSCI, as can occur with monotone dropout. These results shift the burden on investigators from passively invoking MAR to justifying, on substantive grounds, the specific mechanisms it requires. We then consider identification of a target law p(v) of variables V by a MAR-assuming analysis, e.g., multiple imputation, that includes complete auxiliary variables Z (variables not in V). Barring a perfect cancellation, such an analysis recovers p(v) if and only if MAR holds with respect to V and Z jointly. We show that if there exists any set of auxiliaries such that (V, Z) obeys MAR, then the complete candidate auxiliaries that are ancestors of the target variables or their missingness indicators form a sufficient set. Contrary to standard recommendations, not all candidate auxiliaries should be used: even complete auxiliaries can introduce MAR violations that would not otherwise occur. We illustrate these results with simulations and an analysis of sexual identity change in the Stockholm Public Health Cohort, where our results indicate that a candidate auxiliary, income, should be excluded; including it attenuated estimates toward the null.

==> xref_main_labels.tex <==
\makeatletter
\newlabel{main-sec:prelims}{{2}{5}{Preliminaries}{}{}}
\newlabel{main-ass:cc_positivity}{{A1}{6}{Complete-case positivity}{}{}}
\newlabel{main-ass:weak_intersection}{{A2}{7}{Weak intersection with respect to $S$}{}{}}
\newlabel{main-sec:dags}{{2.2}{7}{DAGs representing missing data}{}{}}
\newlabel{main-tb:notation}{{1}{8}{List of key notation}{}{}}
\newlabel{main-sec:MAR_MNAR}{{2.3}{9}{Standard definitions of MAR and MNAR}{}{}}
\newlabel{main-def:eMAR}{{1}{9}{MAR and MNAR}{}{}}
\newlabel{main-eq:mar_ipw_true}{{1}{10}{Standard definitions of MAR and MNAR}{}{}}
\newlabel{main-def:c_inactive}{{2}{10}{c-inactivity}{}{}}
\newlabel{main-fig:c_inactivity_dags}{{1}{11}{Three causal mechanisms that can generate c-inactivity. These are not exhaustive. In each panel, the blue dotted edge $A \to B$ is c-inactive in context $D = d$. (a) $D$ interacts with $A$ in $f_B$ such that $A$ does not affect $B$ when $D = d$. (b) $D$ is not a parent of $B$, but $D = d$ implies $K = k$, and $K$ interacts with $A$ in $f_B$ such that $A$ does not affect $B$ when $K = k$. (c) $D = d$ confines $A$ to values across which $f_B$ does not vary (e.g., a single value)}{}{}}
\newlabel{main-def:pruned_DAG}{{3}{12}{Pruned DAG}{}{}}
\newlabel{main-def:c_faithfulness}{{4}{13}{c-faithfulness}{}{}}
\newlabel{main-fig:monotone_MAR}{{2}{14}{DAGs depicting monotone MAR with no complete variables, with and without pruning. Annotations below edges between members of $R$: determinism due to monotone missingness. Blue dotted edges are annotated with their labels, i.e., contexts in which they are c-inactive; each is also c-inactive in any context that forces the annotated value}{}{}}
\newlabel{main-sec:equivalent_conditions_unrestricted}{{3}{14}{MNAR-equivalent mechanistic conditions}{}{}}
\newlabel{main-def:VMAR}{{5}{14}{}{}{}}
\newlabel{main-def:vmar_violating_path}{{5}{14}{}{}{}}
\newlabel{main-fig:VMAR_VMNAR_examples}{{3}{15}{Variables shaded in gray are incomplete. With $S := L$ and $\{U_1, U_2\}$ latent: (a) each red dotted edge is a VMAR-violating path; and (b) the red dotted path $L_1 \gets U_1 \to L_2 \gets U_2 \to R_{L_1}$ is a VMAR-violating path. (c) is the latent projection (Section \ref {sec:connections_other_lit}) of (b) with $U_1, U_2$ marginalized out}{}{}}
\newlabel{main-def:mar_violating_path}{{6}{16}{MAR-violating paths}{}{}}
\newlabel{main-def:variable_dependence}{{7}{16}{}{}{}}
\newlabel{main-ass:no_csci}{{A3}{16}{No CSCI in missingness contexts with respect to $S$}{}{}}
\newlabel{main-thm:mnar_equivalent}{{1}{17}{MNAR-equivalent conditions}{}{}}
\newlabel{main-fig:mnar_implication_map}{{4}{19}{Implications among MNAR($S$) and related conditions (top) and their negations (bottom). Numbers on edges correspond to parts of Theorem \ref {thm:mnar_equivalent}. Dashed edges require the indicated assumptions: weak int. = weak intersection (Assumption \ref {ass:weak_intersection}); c-faith. = c-faithfulness (Definition \ref {def:c_faithfulness}); CSCI restr. = no CSCI in missingness contexts (Assumption \ref {ass:no_csci}); no canc. = no perfect cancellations in the MAR law (Supplement, Assumption \ref {supp-ass:no_mar_law_cancellations}). Solid edges hold in every compatible SCM obeying complete-case positivity. If $Z$ is a set of complete auxiliary variables and $S := V \cup Z$, then $\pMAR {S}(s) \ne p(s)$ can be replaced by $\pMAR {V \cup Z}(v) \ne p(v)$ in the top panel and $\pMAR {S}(s) = p(s)$ be replaced by $\pMAR {V \cup Z}(v) = p(v)$ in the bottom panel (Corollary \ref {coro:aux_equivalent}); the dashed edge (4) then also requires no perfect cancellations over the auxiliaries (Supplement, Assumption \ref {supp-ass:no_margin_cancellations})}{}{}}
\newlabel{main-coro:incomplete_vars_cant_fix_mnar}{{1}{19}{Incomplete variables cannot restore VMAR}{}{}}
\newlabel{main-sec:connections_other_lit}{{3.1}{20}{Connections to existing literature}{}{}}
\newlabel{main-sec:auxiliaries}{{4}{21}{Identification using auxiliary variables}{}{}}
\newlabel{main-lm:margin_correct}{{2}{21}{Correctness for the target law}{}{}}
\newlabel{main-coro:aux_equivalent}{{1}{21}{MAR-assuming identification with complete auxiliaries}{}{}}
\newlabel{main-sec:constructing_suff_aux_set}{{4.1}{22}{Constructing sufficient auxiliary sets}{}{}}
\newlabel{main-def:suff_aux_set}{{8}{23}{Sufficient auxiliary set}{}{}}
\newlabel{main-thm:suff_set_general}{{2}{23}{A sufficient auxiliary set for partially unknown DAGs}{}{}}
\newlabel{main-fig:suff_aux_set}{{5}{24}{A DAG $G$ illustrating Theorem \ref {thm:suff_set_general}, with target variables $V := \{ V_1, V_2 \}$ and candidate auxiliary variables $W := \{ W_1, W_2 \}$. Gray shading: incomplete variables. Red dotted path: VMAR-violating path when including $W_1$. $U_1$ and $U_2$ are latent}{}{}}
\newlabel{main-sec:practical_implications_aux}{{4.2}{24}{Practical implications}{}{}}
\newlabel{main-sec:applied}{{4.3}{26}{Applied example}{}{}}
\newlabel{main-fig:applied_example_dag}{{6}{26}{DAG $G$ representing the applied example. Gray shading: Incomplete variables. Red dotted path: VMAR-violating path when including income. $\text {ID}_1$: Sexual identity at baseline (exposure; $V_1$). $\text {ID}_2$: Sexual identity at follow-up (outcome; $V_2$). $U_1$: Stigmatization. $U_2$: Parental leave. Sex and income are complete candidate auxiliary variables; $U_1$ and $U_2$ are latent}{}{}}
\newlabel{main-sec:discussion}{{5}{28}{Discussion}{}{}}
\newlabel{main-sec:data-availability}{{5}{31}{Data availability}{}{}}
\makeatother


==> xref_supp_labels.tex <==
\makeatletter
\newlabel{supp-tb:results_index}{{S1}{3}{Index of all theoretical results and their dependencies, i.e., other results or assumptions used to establish the result in the first column. ``Converse'' marks an assumption needed only for the converse direction}{}{}}
\newlabel{supp-fig:proof_dependency_flowchart}{{S1}{4}{Dependency structure of the results}{}{}}
\newlabel{supp-sec:addl_prelims}{{1.1}{5}{Additional preliminaries}{}{}}
\newlabel{supp-def:minimal_vmar_path}{{S1}{5}{Minimal VMAR-violating paths}{}{}}
\newlabel{supp-sec:DAGs}{{1.1.1}{5}{Causal graphs with missing data}{}{}}
\newlabel{supp-def:projection}{{S2}{6}{Latent projection}{}{}}
\newlabel{supp-sec:review_assumptions}{{1.1.2}{7}{Review of assumptions}{}{}}
\newlabel{supp-sec:regularity_assumptions}{{1.1.2}{7}{Review of assumptions}{}{}}
\newlabel{supp-ass:boring_assumptions}{{S0}{7}{Regularity assumptions}{}{}}
\newlabel{supp-ass:no_margin_cancellations}{{S0(i)}{7}{Regularity assumptions}{}{}}
\newlabel{supp-ass:no_mar_law_cancellations}{{S0(ii)}{7}{Regularity assumptions}{}{}}
\newlabel{supp-ass:cc_positivity}{{A1}{7}{Complete-case positivity}{}{}}
\newlabel{supp-ass:weak_intersection}{{A2}{7}{Weak intersection with respect to $S$}{}{}}
\newlabel{supp-sec:csci}{{1.2}{7}{General framework for context-specific causal irrelevance}{}{}}
\newlabel{supp-lm:pruning_soundness}{{S1}{8}{Markov property with c-inactivity}{}{}}
\newlabel{supp-sec:rmm_example}{{1.2.1}{9}{Example: RMM}{}{}}
\newlabel{supp-fig:ex_rmm}{{S2}{10}{Randomized monotone MAR. Gray shading indicates incomplete variables. Bold red edges: determinism. Blue dotted edges are annotated with their labels, i.e., contexts in which they are c-inactive; each is also c-inactive in any context that forces the annotated value. In the context $R_{L_1} = 0$, the edge $L_1 \to R_{L_2}$ is c-inactive, so it is deleted in panel (b)}{}{}}
\newlabel{supp-sec:thm1_proof}{{1.3}{10}{Theorem \ref {main-thm:mnar_equivalent}: MNAR-equivalent conditions}{}{}}
\newlabel{supp-thm:mnar_variable_level}{{1(1)}{10}{MNAR-equivalent conditions: variable-level independences}{}{}}
\newlabel{supp-thm:mnar_mechanistic}{{1(2)}{12}{MNAR-equivalent mechanistic conditions}{}{}}
\newlabel{supp-thm:mnar_paths}{{1(3)}{13}{MAR-violating and VMAR-violating paths}{}{}}
\newlabel{supp-prop:mar_fnl_correct}{{S1}{14}{Correctness of the MAR-assuming functional}{}{}}
\newlabel{supp-prop:minimal_vmar_paths}{{S2}{14}{Minimal VMAR-violating paths in the latent projection}{}{}}
\newlabel{supp-sec:boring}{{1.3.1}{15}{Supporting lemmas}{}{}}
\newlabel{supp-lm:product_support_implies_weak_intersection}{{S2}{15}{Selecting a single member}{}{}}
\newlabel{supp-lm:general_path_truncation_helper}{{S3}{16}{Path truncation helper}{}{}}
\newlabel{supp-sec:aux_results}{{1.4}{17}{Lemma \ref {lm:margin_correct}: Correctness for the target law}{}{}}
\newlabel{supp-lm:margin_correct}{{2}{17}{Correctness for the target law}{}{}}
\newlabel{supp-lm:constructing_a_dsep_set}{{S4}{17}{Conditional d-separating set among a subset of nodes}{}{}}
\newlabel{supp-thm:suff_set_general}{{2}{18}{A sufficient auxiliary set for partially unknown DAGs}{}{}}
\newlabel{supp-fig:mnar_implication_map_with_mealli}{{S3}{19}{Implications among MNAR($S$) and related conditions, with a comparison to Mealli \& Rubin (2015).\autocite {mealli2015clarifying} Numbers on edges correspond to parts of Theorem \ref {main-thm:mnar_equivalent} in the main text. Dashed edges require the indicated assumptions: weak int. = weak intersection (Assumption \ref {ass:weak_intersection}); c-faith. = c-faithfulness (Definition \ref {main-def:c_faithfulness}); CSCI restr. = no CSCI in missingness contexts (Assumption \ref {main-ass:no_csci} in the main text); no canc. = no perfect cancellations in the MAR law (Assumption \ref {ass:no_mar_law_cancellations}). Solid edges hold in every compatible SCM obeying complete-case positivity. The diagonal black edge is the standard result that VMAR($S$) implies MAR($S$) in every compatible SCM (equivalently, MNAR($S$) implies that a VMAR-violating path exists); it is not part of Theorem \ref {main-thm:mnar_equivalent}. Gray: comparison with Theorem 1 of Mealli \& Rubin (2015)\autocite {mealli2015clarifying} (discussed in Section \ref {main-sec:connections_other_lit} of the main text), whose condition is the rightmost node. std.\ faith. = faithfulness of the distribution to $G$; indep.\ $R(S)$ = $R_i \indM (R(S) \setminus \{R_i\}) \mid S$ for all $i$; pos. = $p(R_{S^*} = 0 \mid s) > 0$ wherever the dependence occurs}{}{}}
\newlabel{supp-sec:vmar_vs_colluding}{{2.2}{19}{VMAR-violating paths versus colluding paths}{}{}}
\newlabel{supp-fig:vmar_vs_colluding_G}{{S4a}{20}{$G$}{}{}}
\newlabel{supp-sub@fig:vmar_vs_colluding_G}{{a}{20}{$G$}{}{}}
\newlabel{supp-fig:vmar_vs_colluding_full}{{S4b}{20}{$G(S \cup R(S))$ with $S := V \cup W$}{}{}}
\newlabel{supp-sub@fig:vmar_vs_colluding_full}{{b}{20}{$G(S \cup R(S))$ with $S := V \cup W$}{}{}}
\newlabel{supp-fig:vmar_vs_colluding_empty}{{S4c}{20}{$G(V \cup R(V))$}{}{}}
\newlabel{supp-sub@fig:vmar_vs_colluding_empty}{{c}{20}{$G(V \cup R(V))$}{}{}}
\newlabel{supp-fig:vmar_vs_colluding}{{S4}{20}{Gray shading indicates incomplete variables. Edge types: \textcolor {blue}{dashed blue} = VMAR-violating path with respect to $V$ but not colluding path with respect to $S := V \cup W$; \textcolor {red}{dotted red} = colluding path with respect to $S$ but not VMAR-violating path with respect to $V$; \textcolor {bothColor}{solid green} = both. (a) The DAG $G$. (b) The ADMG $G(S \cup R(S))$ with $S := V \cup W$, where $U_1$ has been marginalized out producing the bidirected edge $V_3 \leftrightarrow R_{V_3}$. (c) The ADMG $G(V \cup R(V))$, where $W_1$ is also marginalized out, producing $V_2 \leftrightarrow R_{V_2}$}{}{}}
\newlabel{supp-sec:rmm}{{3}{21}{Randomized monotone MAR}{}{}}
\newlabel{supp-sec:sim_study}{{4}{22}{Example DAGs and simulation study}{}{}}
\newlabel{supp-sec:examples_sims}{{4.1}{22}{Example DAGs}{}{}}
\newlabel{supp-tb:simulation_dags}{{S2}{22}{Latent projections of DAGs used in the simulation study, illustrating sufficient and insufficient choices of complete auxiliary variables. For compactness, associations caused by latent common causes ($U$) of variables are depicted as bidirected edges}{}{}}
\newlabel{supp-tb:dgp_correlations}{{S3}{24}{Data-generating mechanisms and empirical marginal correlations for simulation scenarios (rounded to two decimals; blank cells indicate $|\rho | < 0.02$)}{}{}}
\newlabel{supp-tb:sim_results}{{S4}{26}{Results}{}{}}
\newlabel{supp-sec:applied}{{5}{27}{Applied example: Changes in sexual identity}{}{}}
\newlabel{supp-tb:applied_var_defns}{{S5}{28}{Variable definitions and sources. Sampling frame was selected from the TPR on 2009-12-31 in SPHC 2010 cohort, and 2014-08-31 in SPHC 2014 cohort. In SPHC 2010, T1 refers to 2010 and T2 to 2014 or 2021; in SPHC 2014, T1 refers to 2014 and T2 to 2021. Abbreviations: CPI, Consumer Price Index; LISA, the Swedish Longitudinal Integrated Database for Health Insurance and Labor Market Studies; PDR, Prescribed Drug Register; SEK, Swedish Krona; SPHC, Stockholm Public Health Cohort; TPR, Total Population Register}{}{}}
\newlabel{supp-tb:baseline_characteristics_1}{{S6}{29}{Characteristics of participants aged 25–45 years with observed sexual identity at baseline in SPHC 2010 cohort. Variable definitions are available in Table \ref {tb:applied_var_defns}. Abbreviations: SD, standard deviation; SEK, Swedish Krona; SPHC, Stockholm Public Health Cohort}{}{}}
\newlabel{supp-tb:baseline_characteristics_2}{{S7}{30}{Characteristics of participants aged 25–45 years with observed sexual identity at baseline in SPHC 2014 cohort. Variable definitions are available in Table \ref {tb:applied_var_defns}. Abbreviations: SD, standard deviation; SEK, Swedish Krona; SPHC, Stockholm Public Health Cohort}{}{}}
\newlabel{supp-tab:imputation_model_summary}{{S8}{32}{Effect estimates by imputation model, stratified by sex. In SPHC 2010 cohort, T1 refers to 2010 and T2 to 2014 or 2021; in SPHC 2014 cohort, T1 refers to 2014 and T2 to 2021. The study samples included participants aged 25 to 45 with observed sexual identity at T1. The substantive analysis model used a log-binomial regression, with sexual identity change (yes vs. no) as the outcome and sexual identity at T1 as the exposure. Missingness in sexual identity at T2 was primarily due to loss to follow-up. \( m \) denotes the number of imputed datasets. Bold indicates the assumed collider variable. Abbreviations: CI, confidence interval; RR, risk ratio; SPHC, Stockholm Public Health Cohort}{}{}}
\newlabel{supp-fig:forest_male}{{S5a}{33}{Among males}{}{}}
\newlabel{supp-sub@fig:forest_male}{{a}{33}{Among males}{}{}}
\newlabel{supp-fig:forest_female}{{\caption@xref {fig:forest_female}{ on input line 20}}{33}{Results}{}{}}
\newlabel{supp-sub@fig:forest_female}{{a}{33}{Results}{}{}}
\newlabel{supp-fig:forest_plots}{{S5}{33}{Estimated associations between non-heterosexual identity at baseline and change in sexual identity at follow-up, presented by cohort and imputation model and stratified by sex. The years in parentheses indicate the follow-up period for each cohort. MICE without income included age, country of birth, antidepressant use, and anxiolytic use as auxiliary variables, whereas MICE with income additionally included income. Abbreviations: CI, confidence interval; MICE, multiple imputation by chained equations; SPHC, Stockholm Public Health Cohort}{}{}}
\newlabel{supp-sec:applied_bias}{{5.4}{34}{Direction of bias from including income}{}{}}
\makeatother

